LP-LLM: End-to-End Real-World Degraded License Plate Text Recognition via Large Multimodal Models

Real-world License Plate Recognition (LPR) faces significant challenges from severe degradations such as motion blur, low resolution, and complex illumination. The prevailing "restoration-then-recognition" two-stage paradigm suffers from a fundamental flaw: the pixel-level optimization objectives of image restoration models are misaligned with the semantic goals of character recognition, leading to artifact interference and error accumulation. While Vision-Language Models (VLMs) have demonstrated powerful general capabilities, they lack explicit structural modeling for license plate character sequences (e.g., fixed length, specific order). To address this, we propose an end-to-end structure-aware multimodal reasoning framework based on Qwen3-VL. The core innovation lies in the Character-Aware Multimodal Reasoning Module (CMRM), which introduces a set of learnable Character Slot Queries. Through a cross-attention mechanism, these queries actively retrieve fine-grained evidence corresponding to character positions from visual features. Subsequently, we inject these character-aware representations back into the visual tokens via residual modulation, enabling the language model to perform autoregressive generation based on explicit structural priors. Furthermore, combined with the LoRA parameter-efficient fine-tuning strategy, the model achieves domain adaptation while retaining the generalization capabilities of the large model. Extensive experiments on both synthetic and real-world severely degraded datasets demonstrate that our method significantly outperforms existing restoration-recognition combinations and general VLMs, validating the superiority of incorporating structured reasoning into large models for low-quality text recognition tasks.

==> sec/5_conclusion.tex <==
\section{Conclusion}
In this paper, we address the problem of license plate recognition under severe degradation by proposing a novel end-to-end paradigm that transcends traditional "image restoration" approaches. We posit that the key to solving recognition under blur lies not in reconstructing perfect pixels, but in reconstructing clear semantic structures within the multimodal feature space. By integrating Qwen3-VL with the newly designed Character-Aware Multimodal Reasoning Module (CMRM), we successfully incorporate strong structural priors of license plates (position, quantity, order) explicitly into the visual encoding process of the large model. The CMRM utilizes a Slot Query mechanism to facilitate a shift from "passive visual perception" to "active character retrieval" and guides the language model to focus on critical character features through a token injection mechanism. Experimental results demonstrate that our method exhibits superior robustness in real-world adverse conditions, significantly outperforming state-of-the-art cascaded super-resolution/deblurring and recognition schemes. This study not only provides an efficient and unified solution for challenging license plate recognition but also serves as a valuable exemplar for integrating domain-specific structured knowledge into general-purpose multimodal large models. Future work will explore the generalization capabilities of this framework in other structured text recognition tasks, such as scene text and document understanding.
